Optimally Summarizing Data by Small Fact Sets for Concise Answers to Voice Queries

Our goal is to find combinations of facts that optimally summarize data sets. We consider this problem in the context of voice query interfaces for simple, exploratory data analysis. Here, the system answers voice queries with a short summary of relevant data. Finding optimal voice data summaries is computationally expensive. Prior work in this domain has exploited sampling and incremental processing. Instead, we rely on a pre-processing stage generating summaries of data subsets in a batch operation. This step reduces run time overheads by orders of magnitude. We present multiple algorithms for the pre-processing stage, realizing different tradeoffs between optimality and data processing overheads. We analyze our algorithms formally and compare them experimentally with prior methods for generating voice data summaries. We report on multiple user studies with a prototype system implementing our approach. Furthermore, we report on insights gained from a public deployment of our system on the Google Assistant Platform.

==> replies.tex <==
Dear reviewers,

\vspace{0.25cm}
we thanks the reviewers for their insightful comments which have helped us to improve the paper significantly. We added eight new examples, new figures, new experiments, more prior work, and we rewrote large parts of the paper. We believe that the revision addresses all points, the changed parts of the paper are marked up in red. Next, we discuss requests by each reviewer and how we addressed them.

\vspace{0.25cm}
\textbf{Meta Review.}

The major points are:
(1) The presentation needs significant improvement (All reviewers).
\begin{answer}
We rewrote significant parts of the paper, adding many new examples and figures.
\end{answer}

(2) The problem statement and details of contributions should be made more clear (Reviewer \#3 and \#4).

\begin{answer}
We clarified the problem statement with various examples and rewrote several parts of the paper to make the contributions more clear.
\end{answer}

(3) Related work needs to be extended (Reviewer \#2).

\begin{answer}
We expanded the related work section.
\end{answer}


(4) Evaluation need to be revised w.r.t metrics but also better explanation of the performance results (Reviewer \#4).

\begin{answer}
We explain performance results in more detail and added more metrics (e.g., latency in Figure~\ref{fig:runTimeOverheads}).
\end{answer}

\vspace{0.25cm}
\textbf{Reviewer \#2. }

D1. Related work should be more extensive covering NL2SQL, data summarization and text generation.

\begin{answer}
We expanded Section~\ref{relatedSec} accordingly.
\end{answer}

D2. The introduction should explain what is the problem that this paper tries to solve specifically, why it is challenging, and what contributions it makes.

\begin{answer}
In the revised introduction, we start by explaining quickly what the problem is, we point out why it is challenging to solve, and enumerate our contributions.
\end{answer}

%the paper essentially focuses on the pre-processing part. It would be useful to elaborate this part of the figure. More specifically, the paper should explain what is happening offline and what is happening at query time (giving a preview for the answers for D4-D7 as well). Use a 

D3. Wrt Figure 1, ... running example ... %with a relation, some facts, some example segments, a user query and returned answers to explain the basic concepts and the workflow of the system,

\begin{answer}
We redid Figure~\ref{overviewFig}, making the connections of the proposed algorithms to the pre-processing part more apparent and showing additional components in pre-processing. We rewrote the system overview section (now Section~\ref{overviewSec}) to provide more details, including one example illustrating the entire workflow at the end of Section~\ref{overviewSec}. 
\end{answer}

D4. The paper needs to clarify how the facts and speeches are generated in the first place. The space of exploration is limited to specific values from the input samples. This poses questions on generalization and scalability aspects.

\begin{answer}
Please note that the space of exploration is not limited by the input samples. For a simple but common class of queries, we pro-actively generate speech summaries for all possible queries up to a certain query length (considering all predicates that can be formed with the values in the database). This generates thousands to ten thousands of speeches for most of the data sets we use for our experiments (see Section~\ref{sub:computational} for precise numbers). We provide details on facts and queries considered in the rewritten Section~\ref{overviewSec}.

We had mentioned a few tens of input samples in the old paper version. However, those samples are only used to train an ML approach to extract constants for query predicate from input text. The resulting extractor has access to all values in the database (i.e., it is not restricted to extracting only constants that appeared in the input samples). Hence, neither the number of queries nor the number of speeches is in any way restricted by the number of extractor training samples.
\end{answer}

D5. At query time, a user query is matched to a pre-defined segment. What if there is no exact match? Is the system willing to give an approximate answer? How does it explain it to the user?

\begin{answer}
The system is willing to give approximate answers. If no speech was generated for the precise input query, the system uses the closest match. The details are outlined in Section~\ref{overviewSec}. Also, the system describes via voice output the query that the voice description refers to. This allows users to interpret the output correctly. 
\end{answer}

D6. If wrt the previous comment, the paper does not do anything more than just returning an exact matching answer, then the paper needs even more to explain the difference to other data summarization works.

\begin{answer}
We go beyond exact matching but have added more details on differences to prior work on data summarization (Section~\ref{relatedSec}).
\end{answer}

D7. Before giving definitions 4 and 5, the paper should motivate why we need it. It just says that we try to model use expectations but I am not sure I understand what that means. It would be useful here to start with an example, explain what is the problem we try to solve and explain how we try to solve it (introducing utilities and deviation, as well as the problem itself).

\begin{answer}
In our revision, we motivate our utility model directly before those definitions. Also, we added various examples, before and after Definitions 4 and 5, illustrating utility and deviation among other things (e.g., Example~\ref{ex:utility}).
\end{answer}

D8. The description of the algorithms is "too low-level". Please introduce each algorithm by giving the big picture first: what the special characteristic of this solution is, and how it works in a few words.

\begin{answer}
We rewrote the beginning of each of the three sections introducing algorithms, explaining what the algorithm does and how it works at a high level.
\end{answer}

D9. It seems odd that the paper first gives a greedy and then an exhaustive solution. Please explain.

\begin{answer}
We changed the order of the sections: the revised version introduces the exhaustive solution first.
\end{answer}

D10. "queries simply describe a data subsets (scope) that is defined" does not read right

\begin{answer}
We replaced that sentence.
\end{answer}

D11. The authors basically compare to their own work. What about other works in data summarization

\begin{answer}
We believe that our own work is closest in terms of focus (generating speech descriptions), objective function (minimizing deviation between expectations and data), and constraints (limit the number of facts). Nevertheless, we added more experiments and expanded our prior work section to include other work on summarization.
\end{answer}

D11. The paper should explain how the crowd workers could tell if a text segment is good or bad, especially assuming they do not know what data is stored in the database.

\begin{answer}
For the experiments reported in Figure~\ref{fig:userPref}, crowd workers compare three alternative summaries describing exactly the same data. The basis of comparison are therefore the alternative descriptions, rather than the raw data. For instance, if they discover facts they find particularly interesting in one speech, it may decrease their rating for others in which it does not appear. Alternatively, if a speech adds facts they consider non-interesting, they can penalize it for lack of conciseness. Making crowd workers aware of all details of the summarized data set is essentially impossible, given that the raw data encompasses hundreds (ACS) or thousands (flights) of rows. However, they get some information on the data via the three summaries. We added a corresponding statement in Section~\ref{sub:userStudies}.

Note that, for the experiments in Figure~\ref{fig:visp}, we use raw data to evaluate speech quality. We compare crowd worker estimates, after them listening to speech descriptions, against actual data. We evaluate speech quality based on how close estimates come to actual values. This setup does not require making crowd workers aware of the data.
\end{answer}

\vspace{0.25cm}
\textbf{Reviewer \#3.}

D1. Regarding W1: Section I is very handwaving and does not tell the reader what is the problem ...

%. Section II provides some irrelevant details, such as the implementation uses Java and Postgres, while it is still totally unclear what the problem is. Section III rushes into formal definitions, again, without telling what the problem is. I was almost ready to reject paper, until I read the last paragraph of Section III, jumped to Table III and Figure 5 in the experiments, and finally figured out what the paper is about. Also, it is uncommon in top conference papers to have a theorem as handwaving as Theorem 4.

\begin{answer}
We bring the problem statement earlier and added various new examples.
\end{answer}

R1. Please explain how the method models the user's prior knowledge. ... %For example, in Figure 5, before listening to the "speeches", the user might already assume that there are much more Elders who have hearing problems that younger people. So, even with the "worst speech", the user might still report a higher number of elders than teenagers.

\begin{answer}\label{an:prior}
In principle, our method can work with any prior, assigning rows to default expectations (our implementation allows any SQL expression to model the prior). In the experiments, we simply use the average value in the target column, averaging over the entire table (e.g., the overall average delay for the data set on flight delays). This assume users have some, but not very detailed, knowledge about realistic values. As shown in Figure~\ref{fig:visp}, when asking users for estimates during our user study, they did indeed report higher values for Elders after listening to the worst speech. Nevertheless, even with a simplifying prior, their estimates came significantly closer to the true values for the speech that is optimal according to our model. We explain how we model the prior in Section~\ref{setupSub}.
\end{answer}

R2. Searching for the "optimal speech" is expensive due to the exponential search space. Can we address the problem with machine learning instead, such as reinforcement learning / evolution methods?

\begin{answer}
We agree that such methods could be used. In fact, the baseline we compare against (Figure~\ref{fig:runTimeOverheads}) uses reinforcement learning (the UCT algorithm, applied to data samples) as well. However, while the search space is exponential, our greedy algorithm has linear complexity in the number of speech facts. Given that it is used before run time, its  overheads seem reasonable in practice. At the same time, it formally guarantees speeches whose utility is within a constant of the theoretical optimum. It seems therefore like a practical option that comes with formal guarantees typical ML methods could not provide. In the revised version, we compare against ML-based data summarization methods in more detail in Section~\ref{relatedSec} and added the requested ML baseline, as described in Answer~\ref{an:ML}, in Section~\ref{sub:vsBaselines}.
\end{answer}

\vspace{0.25cm}
\textbf{Reviewer \#4.}

W1. The paper does not explain the basic concepts clearly. ... %It does not explain what it means by dimensions and target columns. Do dimension columns indicate the columns participating in equality predicates? What is a target column? Does it mean a projected column in a query? Since the definition of a “fact” is based on the dimension and target columns, and the remaining paper is built upon the notion of a “fact”, the remaining paper leads to a painstaking reading experience. It is advised that the definitions in Section 3 are rewritten by using an example for every term. The example of table 3 referred at the end of section 3 is not descriptive enough.

\begin{answer}
In the revised version, we added various examples in the section introducing the problem model (now Section~\ref{modelSec}).
\end{answer}

W2. The paper defines utility of a fact as the deviation between the user expectation and the actual value. ...  Again, an example is needed here.

%The prior expectation by the user before listening to any speech is modeled via a prior function P(r). How is the prior expectation function defined? This is not made clear in the paper. It is crucial to know because, the entire paper pivots on the idea that a minimum number of facts which maximize utility are used to summarize a query answer. Since maximizing utility is all about minimizing the deviation between the user expectation and actual value, the notion of expectation needs to be made clear.

\begin{answer}
We clarify in Section~\ref{setupSub} the prior used in our experiments (we simply used the average value over all rows in the target column). Generally, our method can be used with any prior function (defined in our implementation via an SQL expression). Also, we added Example~\ref{ex:utility} to illustrate how utility is calculated. Please refer to Answer~\ref{an:prior} as well.
\end{answer}

W3. The paper is abstract and vague at several places. For instance, in order to prune facts, the paper comes up with a pair of fact groups – a source fact group and a target fact group. It is unclear why two sets are required here. Can’t we reason with a single fact group which needs to be added incrementally as long as it does not bring the overall utility down? A detailed and an intuitive explanation is required here while clearly stating down the need for two fact groups and what they mean for the solution. Having a running example in the paper and using it as a means to explain the algorithms can be very useful.

\begin{answer}
The greedy algorithm must add the fact with maximal utility gain in each iteration (otherwise, it cannot guarantee a near-optimal solution~\cite{Nemhauser1978}). It is insufficient to add facts that increase utility. We use pruning to discard groups of facts that cannot have maximal utility gain. To decide that, we compare an upper bound on utility gain of a fact group against a lower bound on utility gain. The lower bound is derived from the utility of a second fact group. In the revised version, in Section~\ref{sub:pruningOverview}, we explain the goal and process of fact pruning and provide an example.
\end{answer}

%This may not be a reasonable metric because utility is defined by the paper as the deviation between the actual and expected values. It is obvious that the proposed approaches show a high utility in the experimental results as it is a heuristic that is optimized by its algorithms.

W4. The results shown in Figure 2 plot utility on the y-axis to measure the quality of the approaches. ... The quality needs to be determined by a metric that is not used as a heuristic within the algorithm. For instance, the paper could define the effectiveness of the summaries in terms of conciseness, diversity, and other semantic metric which capture how meaningful the answer is to the question asked by the user.

\begin{answer}
Following your suggestion, we added experiments in which we asked crowd workers to evaluate ``conciseness'' and ``diversity'', among other metrics, comparing speeches generated by our approach and a baseline (see Figure~\ref{fig:vsBaselineUser}). Generally, we validate that our utility metric correlates well with user preferences (see Figure~\ref{fig:userPref}), that it correlates with how much listeners learn about the data (see Figure~\ref{fig:visp}), and that its underlying model is more realistic than alternatives (see Figure~\ref{fig:intuition}). Utility, reported in Figure~\ref{fig:performance}, seems like a reasonable proxy for other desirable properties. The algorithms have been designed for this metric but it is still NP-hard to find optimal speeches. This makes it interesting to assess how close the greedy algorithm comes to the optimum.
\end{answer}

%Also note that we validate our utility metric via user studies in Section~\ref{sub:userStudies}. Essentially, we show that There, we show that our utility metric correlates well with several desirable features. Specifically, we show that users are more likely to associate positive attributes (e.g., ``Good'', ``Informative'') with speeches that have higher utility, according to our model. We also show that users estimate data properties more accurately after listening to high-utility speeches. 

W5. The paper compares its proposed approach to a prior sampling-based approach in Figure 9. It is surprising to see that the paper can outperform a sampling-based approach on latency. This is because, the solution used by the paper does not sample any candidates. Rather, it uses some pruning heuristics. Does this imply that the baseline approach samples too many speech summaries? Also, why are the quality results not shown while comparing the proposed approach to the baseline? The paper also needs to present the time spent in pre-processing by both the approaches and needs to justify why it is okay to have a huge pre-processing cost.

\begin{answer}
Please note: latency, as defined by the prior work~\cite{Trummer2018a}, is time until the system starts speaking (while sampling continues in the background to choose the next sentences). The old figure reported total query processing time. This time determines monetary fees per query on Cloud platforms like the one we run our system on. The baseline uses sampling, at run time, to approximate not the quality of one but of many candidate speeches for the same query. Our new system merely performs a lookup at run time, which is significantly cheaper.

Using a lookup is only possible due to an expensive pre-processing phase. However, pre-processing covers \textbf{all possible queries} of a simple but common class of voice queries, up to a certain query length, considering all predicates that can be formed using any constant in the data. As shown in our experiments (Section~\ref{sub:deployment}), pre-processing covers most voice queries received in practice. Large pre-processing costs seem acceptable as it is only done once and before run time. 

Our utility model assumes that speeches provide specific average values. The baseline only conveys coarse-grained value ranges via speech (to facilitate sampling-based approximation). Hence, we cannot calculate utility for the baseline according to our model. %However, we added experiments comparing speech quality in a user study and clarified the points above in the revised paper.

\textbf{\underline{Following your suggestions}}, we rewrote the comparison (Section~\ref{sub:vsBaselines}), and adapted Figure~\ref{fig:runTimeOverheads}, separating latency from processing time. We outline pre-processing overheads, justify why it seems reasonable, and why we cannot calculate utility for the baseline according to our model. Also, we \underline{provide new experiments} asking crowd workers to compare speech quality instead.

%Please note: latency, as defined by the prior work~\cite{Trummer2018a}, is time until the system starts speaking (while sampling continues in the background to choose the next sentences). Figure~\ref{fig:runTimeOverheads} reports total query processing time instead. This time determines monetary fees per query on Cloud platforms like the one we run our system on. The baseline uses sampling, at run time, to approximate not the quality of one but of many candidate speeches for the same query. Our new system merely performs a lookup at run time, which is significantly cheaper.
\end{answer}

W6. Another interesting alternative here is – a machine learning model (like a neural network) can be trained on several pre-generated pairs of $<$speech fragment, summary$>$ and can be used to predict the summaries for voice queries. ... %How would such model compare to the proposed algorithms in this paper? An experimental comparison would be interesting to see.

\begin{answer}\label{an:ML}
We added a baseline that trains on pairs of speech fragments and summaries in Section~\ref{sub:vsBaselines}. Generally, we expanded Section~\ref{relatedSec} to discuss prior work using ML for data summarization.
\end{answer}

W7. Another question here is about the scalability of the algorithm with increasing dimensions. ... %The paper assumes simple equality predicates. With increasing complexity within the SQL queries, it is clear that the search space of possible facts will blow up exponentially. How will the paper handle them? The scalability results shown in Figure 3 assume the presence of at most 3 dimensions on the X-axis. It is typical that database schemata contain hundreds of columns and several tables. For instance, what happens when the SQL queries consist of several multi-join predicates, group by attributes, aggregate columns etc.? The paper needs to clearly mention the complexity in the schema as well as the complexity in the SQL queries that it currently supports.

\begin{answer}
Please note: the x axis of that figure (Figure~\ref{fig:scalability} in the revision) represents the maximal number of dimensions that can appear \textbf{together in the same sentence} of the speech. It disallows sentences like ``The average delay in Winter, at La Guardia Airport, in the morning, for Delta Airlines is 5 minutes'' that are inconvenient to listen to. The total number of dimensions in the table can be much higher, we use up to 7 dimension in our experiments (see Table~\ref{dataSetsTable}). More generally, our approach is optimized for handling queries that are rather short and simple. We hypothesized that it is difficult to convey more complex queries via voice input. We make that point more clear in the revised Section~\ref{overviewSec}. We found our hypothesis to be largely justified (e.g., see Figure~\ref{fig:queryComplexity}) in our user studies. We clarified the set of considered queries in Section~\ref{overviewSec}. 

Scaling: if we can form $n$ predicates on each column, the table contains $d$ columns, and facts reference $3$ of them, then the number of facts is in $O(n^3\cdot d^3)$ (i.e., polynomial growth in the number of table dimensions for constant dimensions per fact). We expanded Section~\ref{analysisSec} with a tighter analysis of how the number of facts and queries depends on the table dimensions.
\end{answer}

%\begin{answer}Our approach is targeted primarily at voice queries. In our experience, it is close to impossible to describe very complex SQL queries via voice input. We performed multiple user studies and analyzed logs recording interactions by various users of our public deployment. Those users were not made aware of the range of supported queries, prior to using the system. In all those cases, we never encountered voice input translating into queries with more than three predicates. While supporting written queries is harder, we believe that our approach is well suited for voice querying. We outlined those points in more detail in Section~\ref{} TODO!!!\end{answer}

==> sections/approximate.tex <==

The algorithm discussed in the previous section does not scale to long speeches and large data sets. We verify this formal results from Section~\ref{exactComplexitySub} empirically in Section~\ref{experimentsSec}. Hence, we discuss a more efficient alternative in the following. We describe the algorithm in Section~\ref{greedySub} and a refinement in Section~\ref{factsSub}. 

\subsection{Greedy Algorithm}
\label{greedySub}

\begin{algorithm}
\renewcommand{\algorithmiccomment}[1]{// #1}
\begin{algorithmic}[1]
\State \Comment{Generate summaries of length $sl$ for relation $R$ with}
\State \Comment{query scope groups $QSG$ and fact scope groups $FSG$.}
\Function{SummarizeApp}{$R,QSG,FSG,sl$}
\State \Comment{Initialize final set of speech summaries}
\State $S\gets\emptyset$
\State \Comment{Iterate over query scope groups}
\For{$qsg\in QSG$}
\State \Comment{Initialize best speeches}
\State $B\gets$ set of empty speeches for each scope in $qsg$
\State \Comment{Get facts for current query scopes}
\State $F\gets$\Call{GenerateFacts}{$R,qsg,FSG$}
\State \Comment{Expand speeches by adding interesting facts}
\For{$i\gets1,\ldots,sl$}
\State \Comment{Expand speeches by relevant facts}
\State $E\gets \{\langle b,f\rangle|s\in B,f\in F:b.scp\subseteq f.scp\}$
\State \Comment{Keep best speech per query scope}
\State $B\gets$\Call{PruneSpeeches}{$R,E$}
\EndFor
\State \Comment{Add final speeches for current scopes}
\State $S\gets S\cup B$
\EndFor
\State \Return{$S$}
\EndFunction
\end{algorithmic}
\caption{Expand speeches greedily by adding most interesting facts until the maximal speech length is reached.\label{approxAlg}}
\end{algorithm}

The number of possible speeches grows exponentially in the speech length. Any algorithm that enumerates all possible speeches therefore scales poorly. Algorithm~\ref{approxAlg} expands speeches greedily instead. Input and output parameters remain the same, compared to Algorithm~\ref{exactAlg}. Algorithm~\ref{approxAlg} iterates again over query scope groups. At the end of each iteration (of the outer loop from Line~7 to 21), a speech has been selected for each scope in the current group. The algorithm reuses auxiliary functions introduced in Algorithm~\ref{auxBasicAlg}. Instead of exhaustive search, it iteratively expands speeches by single facts. In each iteration (of the inner loop from Line~13 to 18), it greedily adds the ``most informative'' fact. The most informative fact is the one that reduces user estimation error maximally. Corresponding speeches can be determined using Function~\textproc{PruneSpeeches}. In the next subsection, we prove that this seemingly simple algorithm guarantees near-optimal speeches in many scenarios.

\subsection{Analysis of Optimality}
\label{greedyOptimalitySub}

We prove in the following that the reduction in estimation error, as a function of speech facts, is sub-modular~\cite{Nemhauser1978}. Intuitively, this means that hearing new facts becomes less interesting, the more we already know. Based on that property, we prove that the greedy algorithm guarantees near-optimal speeches. First, we give a formal definition of sub-modularity.

\begin{definition}
A set function $f:S\mapsto\mathbb{R}^+$ is sub-modular if for all sets $S_1,S_2\subseteq S$ where $S_1$ is a subset of $S_2$ ($S_1\subseteq S_2$), the increase by adding a new element $s\in S$ is higher for $S_1$ than for $S_2$: $f(S_1\cup\{s\})-f(S_1)\geq f(S_2\cup\{s\})-f(S_2)$.
\end{definition}

Next, we analyze error reduction according to different user models.

\begin{theorem}
Error reduction according to the typical value model, as a function of speech facts, is sub-modular.\label{avgTheorem}
\end{theorem}
\begin{proof}
Let $S_1$ and $S_2$ two speeches (sets of average facts) describing the same data such that $S_1\subseteq S_2$. Denote by $s$ a relevant fact that neither appears in $S_1$ nor $S_2$. 
For a fixed row $r$ with dimension values $D_r$ and target value $v_r$, it is $\mathcal{E}_T(S_1)=\min_{\langle D,v \rangle\in S_1:D\subseteq D_r}|v-v_r|\geq \min_{\langle D,v \rangle\in S_2:D\subseteq D_r}|v-v_r|=\mathcal{E}_T(S_2)$ since $S_1\subseteq S_2$. Denote by $\Delta(S,s)=\mathcal{E}_T(S)-\mathcal{E}_T(S\cup\{s\})$ the error reduction by adding fact $s$. We distinguish two cases: either the new fact $s$ provides a better approximation than any fact in $S_2$ (case 1) or not (case 2). In case 1, $s$ provides a better approximation than any fact in $S_1$ as well (since $S_1\subseteq S2$). Hence, $\mathcal{E}(S_1\cup\{s\})=\mathcal{E}(S_2\cup\{s\})$ and $\Delta(S_1,s)\geq \Delta(S_2,s)$ (i.e., error reduction is sub-modular) since $\mathcal{E}_T(S_1)\geq \mathcal{E}_T(S_2)$. In case 2, we have $\Delta(S_2,s)=0$ and therefore $\Delta(S_1,s)\geq \Delta(S_2,s)$ (as error reduction is non-negative). Error is aggregated as the sum over multiple rows. The sum of sub-modular functions (with positive weights) is sub-modular~\cite{Krause2012}.
\end{proof}

\begin{theorem}
Error reduction according to the value range model is sub-modular.\label{rangeTheorem}
\end{theorem}
\begin{proof}[Sketch]
Let $S_1$ and $S_2$ again denote two speeches such that $S_1\subseteq S_2$ and $s\notin S_1,S_2$ a new fact. For a row with target value $v_r$ and dimension values $D_r$, it is $\mathcal{E}_R(S)=(\min_{\langle l,u,D\rangle:D\subseteq D_r}u)-(\max_{\langle l,u,D\rangle:D\subseteq D_r}l)$. We can apply a similar reasoning as in the previous proof, distinguishing the case that the newly added fact shrinks the range between minimum and maximum from the case that it does not. For upper and for lower bound, knowing more facts beforehand can only decrease the impact of the newly added fact. Hence, the error reduction is sub-modular again.
\end{proof}

Based on that property, we can prove that Algorithm~\ref{approxAlg} produces near-optimal speeches.

\begin{theorem}
Algorithm~\ref{approxAlg} produces speeches reducing error within factor $(1-1/e)$ of the optimum.
\end{theorem}
\begin{proof}
Error reduction is non-negative and monotone. Furthermore, we have proven in Theorems~\ref{avgTheorem} and \ref{rangeTheorem} that error reduction is sub-modular. Algorithm~\ref{approxAlg} greedily selects a bounded number of facts for each scope. Doing so guarantees the postulated optimality factor~\cite{Nemhauser1978}.
\end{proof}

\subsection{Complexity Analysis}
\label{greedyComplexitySub}

We show that the greedy algorithm reduces space and time complexity, compared to the exhaustive algorithm. We make the same assumptions and use the same symbols as in Section~\ref{exactComplexitySub}. 

\begin{theorem}
Algorithm~\ref{approxAlg} is in $O(spg\cdot fps\cdot rps)$ space.\label{greedySpaceTheorem}
\end{theorem}
\begin{proof}
Using a similar reasoning as in the proof of Theorem~\ref{exactSpaceTheorem}, the data structure with dominant space requirements pairs rows and partial speeches with new facts. We consider up to $spg$ scopes per group, $fps$ facts per scope, and $rps$ rows per scope. 
\end{proof}

\begin{theorem}
Algorithm~\ref{approxAlg} is in $O(sgs\cdot sl\cdot spg\cdot rps\cdot fps)$ time.\label{greedyTimeTheorem}
\end{theorem}
\begin{proof}
We iterate over $sgs$ scope groups. For each scope group, we expand corresponding speeches $sl$ times (adding facts one by one). To expand speeches, we join relation rows with facts, the join output cardinality is in $O(spg\cdot rps\cdot fps)$. This is the operation with dominant complexity.
\end{proof}

Based on this analysis, we expect the greedy algorithm to scale to significantly larger problems than the algorithm from the previous section. We verify this intuition in our experiments. 

==> sections/exact.tex <==

We describe an algorithm for generating guaranteed optimal speech summaries in Section~\ref{exactAlgSub}. We analyze its complexity in Section~\ref{exactComplexitySub}. 

\subsection{Algorithm}
\label{exactAlgSub}

Our goal is to generate optimal speech descriptions for a large data set, considering all possible query scopes. Each scope is defined by a conjunction of equality predicates on dimension columns. We can treat query scopes separately. More precisely, we can iterate over all query scopes, retrieve rows that fall within the scope, and generate an optimal speech. This is however inefficient as the number of scopes is typically large, requiring many passes. Instead, we present an algorithm that batches query scopes into groups. This algorithm only requires one pass over the input data per scope group.


\begin{algorithm}[t]
\renewcommand{\algorithmiccomment}[1]{// #1}
\begin{algorithmic}[1]
\State \Comment{Generate summaries of length $sl$ for relation $R$ with}
\State \Comment{query scope groups $QSG$ and fact scope groups $FSG$.}
\Function{SummarizeOpt}{$R,QSG,FSG,sl$}
\State \Comment{Initialize final set of speech summaries}
\State $S\gets\emptyset$
\State \Comment{Iterate over query scope groups}
\For{$qsg\in QSG$}
\State \Comment{Get facts for current query scopes}
\State $F\gets$\Call{GenerateFacts}{$R,qsg,FSG$}
\State \Comment{Combine facts into speech candidates}
\State $C\gets\{\langle f_1,\ldots,f_{sl}\rangle|f_i\in F,\text{$f_i$ compatible}\}$ % f_i.scp=f_j.scp\forall i,j
\State \Comment{Add optimal speeches for current scopes}
\State $S\gets S\cup$\Call{PruneSpeeches}{$R,C$}
\EndFor
\State \Return{$S$}
\EndFunction
\end{algorithmic}
\caption{Consider all possible speeches and select optimal summary for batches of query scope.\label{exactAlg}}
\end{algorithm}

We group query scopes that are characterized by restrictions on the same dimension columns. We describe such scope groups by the set of columns. Each group contains all query scopes that restrict each of those columns to a value. The number of scopes per group is therefore determined by the number of unique value combinations (in the input data) for the scope columns. Our choice of scope groups is motivated by our goal of executing the algorithm inside of a relational DBMS. If scope groups are defined by columns, aggregates for all scopes in a group can be efficiently calculated via group by queries.

%We justify this choice of scope groups later in this subsection.

Algorithm~\ref{exactAlg} generates optimal speech descriptions for all query scopes. As input, it obtains the relation $R$, the set $QSG$ of query scope groups (each group is specified as a set of dimension columns), the set $FSG$ of fact scope groups, and the maximal speech length $sl$ (measured as the number of facts). The output is a data structure associating query scopes with optimal speeches. 
The algorithm iterates over all scope groups. It executes three steps for each scope group. First, it generates facts that are relevant for some of the scopes in this group. Second, it combines those facts into speeches up to the specified speech length (only pairing facts that are ``compatible'', meaning that they describe data within the same scope). Finally, it identifies the optimal speech for each scope. The algorithm uses several auxiliary functions that are discussed next. 


%We choose to group query scopes based on their restricted columns for the following reason. For any unique value combination in the scope group columns, the group contains only one scope. Hence, each row in the input data set falls into exactly one scope per group. No row is read in vain when passing over the data since each row will be processed for the current scope group. Also, 


\begin{algorithm}[t]
\renewcommand{\algorithmiccomment}[1]{// #1}
\begin{algorithmic}[1]
\State \Comment{Generate facts on data in $R$ within query scopes $qsg$}
\State \Comment{using relevant fact scopes in $FSG$.}
\Function{GenerateFacts}{$R,qsg,FSG$}
\State \Comment{Basic version: consider all relevant facts}
\State \Return{$\cup_{fsg\in FSG:qsg\subseteq fsg}(\Gamma_{fsg,avg(r.tcol)}(r\in R))$}
\EndFunction
\vspace{0.15cm}
\State \Comment{Compare how well speeches $S$ describe data $R$}
\State \Comment{and keep only best speech for each scope.}
\Function{PruneSpeeches}{$R,S$}
\State \Comment{Pair each data row with associated speech}
\State $P\gets\{\langle r,s\rangle|s.scp\subseteq r.dimVals\}$
\State \Comment{Calculate error of each speech over all rows}
\State $Err\gets\Gamma_{s,sum(|r.tcol-\mathcal{U}(s,r)|)}(\langle r,s\rangle\in P)$
\State \Comment{Return non-dominated speeches}
\State \Return{$\{s|\nexists \langle \widetilde{s},\widetilde{\varepsilon}\rangle\in Err:s.scp=\widetilde{s}.scp,\widetilde{\varepsilon}<\varepsilon\}$}
\EndFunction
\end{algorithmic}
\caption{Auxiliary functions for generating facts and pruning speech summaries.\label{auxBasicAlg}}
\end{algorithm}

Algorithm~\ref{auxBasicAlg} presents several auxiliary functions that are used by Algorithm~\ref{exactAlg} (but also by the algorithms presented in the following sections). Function~\textproc{GenerateFacts} generates relevant facts for the current scope group. As written in pseudo-code, the function generates facts about average values in the target column for different fact scopes. Our actual implementation supports a more diverse set of facts (e.g., facts about minima and maxima value for data subsets). Each fact scope is defined by a conjunction of equality predicates on the dimension columns. A fact scope group contains scopes restricting the same columns. 


Given a query scope, a fact scope is relevant if it describes a subset of data within the query scope. We say that the fact scope specializes the query scope in that case (i.e., the set of predicates characterizing the query scope is a subset of the fact scope predicates). We assume that the set of considered fact scopes is a superset of the set of query scopes. Hence, there is no need to pick a fact scope that is less specific than the current query scope. The constraints connecting (fact and query) scopes translate into constraints on scope groups as follows. 

\begin{lemma}
If $qsg\subseteq fsg$, for a query scope group with columns $qsg$ and fact scope group $fsg$, then every fact in $fsg$ is relevant for some scope in $qsg$.
\end{lemma}
\begin{proof}
Scopes are defined by equality predicates on all scope group columns. Each fact scope restricts all columns in $fsg$. By dropping all predicates associated with columns not in $qsg$, we obtain a predicate subset. All remaining predicates refer to columns in $qsg$ as $qsg\subseteq fsg$. The conjunction of predicates describes a query scope for which the initial fact is relevant.
\end{proof}

Function~\textproc{GenerateFacts} generates facts that are relevant for at least one scope in any of the current query scope groups. Function~\textproc{PruneSpeeches} discards speeches that are sub-optimal. Each speech is evaluated by how well it summarizes data in the corresponding scope. For each pair of a relation row and an associated speech, we calculate the error. The error is the distance between that row's actual value in the target column and an estimate based on the speech. As discussed in Section~\ref{modelSec}, this estimate is calculated using our user model. It represents the value in the target column a user would guess, based on the speech description and the row dimension values. We measure the quality of each speech for each query scope by aggregating per-row error over all rows in that query scope. For each query scope, we only keep the optimal speech.

We execute all steps of the algorithm as SQL queries in a relational DBMS. For instance, generating facts entails group by queries. Facts can be combined into speeches via joins. Also, those speeches are paired with input data using joins. The accumulated error for specific query scopes and speeches is calculated via group by queries. Implementing all steps inside the DBMS avoids costly data movements. Still, the algorithm is simple and does not scale to large data sets (as shown in more detail in the next subsection).

\subsection{Complexity Analysis}
\label{exactComplexitySub}

\begin{table}[t]
\caption{Summary of symbols used for analysis.\label{symbolsTable}}
\begin{tabular}{ll}
\toprule[1pt]
\textbf{Symbol} & \textbf{Semantics}\\
\midrule[1pt]
$sgs$ & Number of scope groups \\
\midrule
$spg$ & Maximal number of scopes per group \\
\midrule
$fps$ & Maximal number of facts per scope \\
\midrule
$rr$ & Number of rows in relation to summarize \\
\midrule
$rps$ & Maximal number of relation rows per scope \\
\bottomrule[1pt]
\end{tabular}
\end{table}

Next, we analyze time and space complexity of Algorithm~\ref{exactAlg}. The symbols introduced in the following are summarized in Table~\ref{symbolsTable} (and are reused in later sections). We denote by $sgs$ the number of scope groups, by $spg$ the maximal number of scopes per scope group, and by $fps$ the maximal number of facts per scope. Parameter $rps$ designates the maximal number of relation rows per scope and $rr$ the total number of relation rows. The maximal number of facts per speech (speech length) is given by $sl$. To simplify the following analysis, we consider cardinality but not the (byte) size per row. Also, we neglect space required for storing the final result (all approaches compared in this paper generate one speech for each scope as final output). 

\begin{theorem}
Algorithm~\ref{exactAlg} is in $O(spg\cdot fps^{sl}\cdot rps)$ space.\label{exactSpaceTheorem}
\end{theorem}
\begin{proof}
We have at most $fps$ facts per query scope. Hence, we can combine $O(fps^{sl})$ speeches of length $sl$ per scope. We treat $O(spg)$ scopes per iteration. Hence, we store $O(spg\cdot fps^{sl})$ speeches. The data structure with dominant space requirements pairs speeches with relation rows. Clearly, it has cardinality $O(spg\cdot fps^{sl}\cdot rr)$. We can refine that to $O(spg\cdot fps^{sl}\cdot rps)$ since each speech applies to only one scope (and we have $O(rps)$ rows per scope). 
\end{proof}

We analyze time complexity under the assumption that the algorithm is executed on top of a relational database management system.

\begin{theorem}
Algorithm~\ref{exactAlg} is in $O(sgs\cdot spg\cdot fps^{sl}\cdot rps)$ time.\label{exactTimeTheorem}
\end{theorem}
\begin{proof}
Algorithm~\ref{exactAlg} combines facts into speeches and pairs speeches with relation rows. This can be realized by joins if data is stored in a relational database. Facts and speeches are paired that refer to the same scope. This can be represented by a conjunction of equality join conditions (on the dimension columns). Hence, join algorithms (e.g., hash joins) with linear complexity in input and output size can be used. The last join in each iteration pairs speeches with data and has dominant time complexity. Its input cardinality is in $O(rr+spg\cdot fps^{sl})$, its output cardinality in $O(spg\cdot fps^{sl}\cdot rps)$ and dominant. The time for identifying the optimal speech per scope is proportional to the latter output cardinality. As we perform $sgs$ iterations, the postulated complexity follows.
\end{proof}

Based on that analysis, finding optimal speech summaries does not scale in the speech length (parameter $sl$). This motivates the algorithm proposed in the next section.

==> sections/experiments.tex <==

We evaluate the proposed approach experimentally. We describe data sets and implementations used for the following experiments in Section~\ref{setupSub}. In Section~\ref{performanceSub}, we report performance results, comparing different voice interfaces in terms of efficiency. In Section~\ref{userSub}, we evaluate our voice interface in several user studies, in comparison to different types of visual interfaces.

\subsection{Experimental Setup}
\label{setupSub}

\begin{table}[t]
\caption{Overview of data sets used for experiments.\label{dataSetsTable}}
\begin{tabular}{p{2cm}p{1.5cm}p{1.5cm}p{1.75cm}}
\toprule[1pt]
\textbf{Data Set} & \textbf{Size} & \textbf{\#Dims} & \textbf{\#Targets}\\
\midrule[1pt]
ACS NY & 2~MB & 3 & 6\\
\midrule
Stack Overflow & 197~MB & 7 & 6 \\
\midrule
Flights & 565~MB & 6 & 1 \\
\midrule
Primaries & 6~MB & 5 & 1\\
\bottomrule[1pt]
\end{tabular}
\end{table}

Table~\ref{dataSetsTable} summarizes the data sets used for the following experiments. We consider an extract from the American Community Survey (prepared for us by the NYC Mayor's Office for People with Disabilities for an upcoming demo on the NYC Open Data week), results of the 2019 Stack Overflow Developer survey\footnote{\url{https://insights.stackoverflow.com/survey/2019}}, a data set on flight delays\footnote{\url{https://www.kaggle.com/usdot/flight-delays}} (frequently used to evaluate OLAP interfaces~\cite{Trummer2018a}), and a data set on the democratic primaries\footnote{\url{https://data.fivethirtyeight.com/}}. Table~\ref{dataSetsTable} reports the number of dimensions and the number of target columns (generating speech summaries for different target columns is done separately, hence the following plots report results of 14 test cases). For the following figures, we report results for data sets in the order in which they are given in Table~\ref{dataSetsTable}. We generate speeches containing up to three (typical value) facts. Query scopes have up to two predicates while fact scopes have up to three predicates. When forming fact scopes, we considered all combinations of dimension columns for each data set. The only exception is the primaries data set where we require fact scopes to contain a restriction on the candidate (thereby preventing the system from averaging votes over multiple candidates which is not informative). For the user studies, a publicly available version of the voice interface was used that can be accessed via smart phones (and other devices supporting the Google Assistant). All of the following performance experiments were executed on a MacBook Air laptop with 8~GB main memory and 1.8 GHz Intel Core i5 CPU. Postgres~11.5 was used as relational processing engine. We configured the maximal speech length to three facts, a value that seems reasonable given limitations of the human short term memory~\cite{Cowan2010}. 

\subsection{Performance Comparisons}
\label{performanceSub}

\begin{figure}[t]
\centering
\begin{tikzpicture}
\begin{groupplot}[group style={group size=1 by 2, x descriptions at=edge bottom}, xlabel={Data Sets}, xlabel near ticks, ylabel={Time (rel.)}, width=8cm, height=3.5cm, ybar=0pt, legend entries={Optimal Speech Summarization}, legend to name={exactTimeLegend}, legend columns=1, ymajorgrids, xmajorticks=false]
\nextgroupplot[title={Relative overheads of exact optimization}, bar width=2.5pt]
\addplot table[x index=0, y index=1, header=false] {plots/exact.txt};
\nextgroupplot[title={Percentage of scope groups causing timeouts}, bar width=2.5pt, ylabel={T-outs (rel.)}]
\addplot table[x index=0, y index=1, header=false] {plots/exactouts.txt};
\end{groupplot}
\end{tikzpicture}

\ref{exactTimeLegend}
\caption{Performance of exhaustive optimization, relative to approximation.\label{exactTimeFig}}
\end{figure}

First, we compare the exhaustive algorithm from Section~\ref{exactSec} against the approximation schemes (Section~\ref{greedySec}). For the exhaustive algorithm, we set a timeout of 30 seconds per query scope group. Figure~\ref{exactTimeFig} shows relative speech generation time (top), scaled to the minimal time per data set (over all compared baselines). The lower part of the figure shows the percentage of query scopes for which the exhaustive algorithm had timeouts. Clearly, exhaustively exploring the space of speech summaries is often significantly (orders of magnitude) more expensive than approximation (which took up to 40 minutes per target column and data set). Relative overheads seem to decrease (upper part of Figure~\ref{exactTimeFig}) for the Stack Overflow developer survey and the flights data. As the lower part of Figure~\ref{exactTimeFig}, this comes however at the expense of a 100\% timeout rate (the two aforementioned data sets are larger and the timeout therefore closer to the time needed by approximate processing). In summary, exhaustively exploring the space of all speeches is prohibitively expensive.



\begin{figure}[t]
\centering
\begin{tikzpicture}
\begin{groupplot}[group style={group size=1 by 1, x descriptions at=edge bottom}, xlabel={Query Scopes}, xlabel near ticks, ylabel={Information}, width=8cm, height=3.5cm, ybar=0pt, legend entries={Approximate Speech Summarization, Theoretical Guarantees}, legend to name={approximateErrorLegend}, legend columns=3, ymajorgrids, xmajorticks=false, ymin=0]
\nextgroupplot[bar width=2.5pt]
\draw[red, ultra thick] (axis cs:1,0.66) -- (axis cs:8,0.66);
\addplot coordinates {(1, 0.99759641177445419356) (2,1) (3,0.99759641177445419356) (4,0.98353724418066794115) (5,0.72765418744681899683) (6,1) (7,1) (8,0.78685707425397191582)};
\end{groupplot}
\end{tikzpicture}

\ref{approximateErrorLegend}
\caption{Error reduction by speeches generated by approximate optimization, relative to optimal reduction. The red line marks the theoretical lower bound due to submodularity.\label{approximatetErrorFig}}
\end{figure}

Next, we analyze the quality of speeches generated by the greedy approach. For comparison, we use the (few) query scopes for which the exhaustive algorithm finishes processing. Figure~\ref{approximatetErrorFig} reports the relative reduction in error by generated speeches (comparing the speech-based estimate for the target column to the default estimate). The red line marks the theoretical minimum (see Section~\ref{greedyOptimalitySub}). A relative reduction of close to one shows that approximate speeches are in most cases near-equivalent to optimal speeches. In any case, the theoretical lower bound of 66\% is achieved.

\begin{figure}[t]
\centering
\begin{tikzpicture}
\begin{groupplot}[group style={group size=1 by 1, x descriptions at=edge bottom}, xlabel={Data Sets}, xlabel near ticks, ylabel={Time (rel.)}, width=8cm, height=3.5cm, ybar=0pt, legend entries={No pruning, Naive, Optimized}, legend to name={compressionLegend}, legend columns=3, xmajorticks=false, ymajorgrids]
\nextgroupplot[bar width=2.5pt]
\addplot table[x index=0, y index=1, header=false] {plots/none.txt};
\addplot table[x index=0, y index=1, header=false] {plots/naive.txt};
\addplot table[x index=0, y index=1, header=false] {plots/opt.txt};
\end{groupplot}
\end{tikzpicture}

\ref{compressionLegend}
\caption{Comparison of execution time for different fact pruning methods.\label{pruningFig}}
\end{figure}

Next, we compare the different variants of the greedy algorithm, discussed in Section~\ref{optimizationSec}. Figure~\ref{pruningFig} compares relative time without fact pruning, with naive fact pruning (i.e., we prune at every occasion), and with optimized pruning. Clearly, no and naive pruning lead to significant overheads in certain scenarios. Naive pruning leads to overheads if pruning is ineffective, while creating large overheads. Among all approximate baselines, it incurred the highest overheads per column and data set (40 minutes for one target column of the Stack Overflow survey). No pruning leads to sub-optimal performance if the number of relevant facts is large, compared to the data set size. Using the optimizer, performance always remains close to the optimum. This shows that our simplifying cost model (see Section~\ref{costSub}) as well as the heuristic restrictions of the plan space (see Section~\ref{plansSub}) are reasonable. While pre-processing is expensive, run time overheads are negligible (selecting speeches for a given query scope corresponds to a simple lookup in a hash table). We store generated speeches as text, resulting in speech summaries of up to 700~KB per column (for columns of the Stack Overflow survey). Further compression is of course possible (storing values instead of text). However, this did not seem necessary for the scenarios we consider.

\subsection{User Studies}
\label{userSub}

The goal of this work is not to replace visual by voice interfaces. Instead, the goal is rather to address scenarios in which visual interfaces are unavailable. Nevertheless, it is interesting to compare voice interfaces against visual interfaces, the dominant type of query interfaces nowadays. We did so in two user studies: one on-site study and a study with crowd workers. 

\begin{figure}
\centering
\begin{tikzpicture}
\begin{axis}[width=8cm, height=3.5cm, ybar=0pt, legend entries={Voice, Visual}, legend columns=2, legend to name=prefLegend, ymajorgrids, xticklabels={U1, U2, U3, U4}, xtick={1,...,10},
  x tick label style={rotate=0}]
\addplot coordinates {(1,3) (2,3) (3,3) (4,2)};
\addplot coordinates {(1,9) (2,5) (3,8) (4,9)};
\end{axis}
\end{tikzpicture}

\ref{prefLegend}
\caption{User preferences comparing visual and voice interfaces (crowd study).\label{crowdPreferences}}
\end{figure}

First, we discuss the results of the crowd study. We used Amazon Mechanical Turk as crowd sourcing platform. Crowd workers were asked to compare two interfaces for data analysis: the voice interface, accessible on all devices running Google Assistant by speaking a key phrase, and the Chart Studio by plotly\footnote{\url{https://plot.ly/chart-studio/}}. Crowd workers were given access to the 2019 Stack Overflow developer survey (the crowd interface contained a link to that data set for import in Chart Studio). We asked them to explore the data and to report interesting trends, as well as for their impression concerning the two interfaces. We paid 50 cents per task and promised an additional bonus of five dollars if crowd workers submitted proof that both interfaces were used at least once (for the voice interface, we asked crowd workers to transcribe the greeting message, we also asked them to upload a screenshot of Chart Studio). We submitted ten HITs on a Wednesday evening (Eastern Time), and ten more HITs on a Friday morning, requiring a minimal HIT acceptance rate of 75\%. We received seven submissions in total, four of which contained the requested proof of having used both interfaces. Most importantly, we asked crowd workers to rate both interfaces on a scale from one to ten (together with the reasons for their rating). 

Figure~\ref{crowdPreferences} reports the results. Surprisingly, the four crowd workers seemed to prefer the voice interface by large margins. Crowd workers cited ease of use as reason to prefer the voice interface (``Direct and to the point. It gave me my answer in seconds.'' to quote one of the crowd workers). The user with the lowest rating for the voice interface hinted at difficulties in speech recognition. A likely explanation seemed to be that crowd workers have no prior experience with data analysis interfaces. Hence, we decided to make a follow-up on-site study, pairing participants with a data analysis interface they are familiar with. More precisely: we paired top-performing students of a database course, focused on SQL, with an SQL query interface. 

The goal of the on-site study was to compare the voice interface, accessed via smart phone, against an SQL interface (Postgres via the psql console). We were able to recruit four participants by soliciting applications from the 15 best students of last semester's database course (a course with about 3,00 students that heavily focuses on SQL). At the beginning of each study, participants were given an introduction to the two interfaces (in particular: the voice interface). Then, we asked participants to explore trends on job satisfaction or salary in the 2019 Stack Overflow Developer Survey with specific interfaces. We gave participants five minutes per data set and interface. After exploration, we asked participants to estimate average values for five data subsets (e.g., we asked them to estimate the average salary for men). Questions were selected by picking random dimensions and values in the respective data with uniform random distribution. By comparing estimation error, we hoped to gain a better understanding of the pros and cons of voice and visual interfaces. Finally, we asked participants for their preferences with regards to the two interfaces. Each study took between 60 and 80 minutes per participant. Participants were rewarded with \$40 per person. 

\begin{table}
\centering
\caption{Relative estimation error (lower is better) and ratio of correctly predicted trends (higher is better) for visual and voice interfaces.\label{userPrecisionTable}}
\begin{tabular}{llll}
\toprule[1pt]
\textbf{Data Set} & \textbf{Metric} & \textbf{Visual} & \textbf{Voice} \\
\midrule[1pt]
Salary & Error & 30\% & 54\% \\
\midrule
& Trends & 72\% & 66\% \\
\midrule
Job satisfaction & Error & 4\% & 5\% \\
\midrule
& Trends & 90\% & 88\% \\
\bottomrule[1pt]
\end{tabular}
\end{table}

Table~\ref{userPrecisionTable} summarizes estimation precision after analyzing data with different interfaces. We report the relative estimation error as well as the percentage of accurate trends, predicted by the participants. For calculating the latter, we compare the five answers per interface and data set pairwise, counting the number of cases in which relative trends of estimates and actual data are consistent. As expected, visual interfaces enable users to explore data at a higher degree of detail. Hence, estimates based on visual analysis are more precise. On the other side, the precision gap is not excessive (e.g., increase between 2 and 9\% of accurately predicted trends). It seems that voice interfaces are able to provide users with a reasonable first impression of data. In any case, precision in predicting relative trends is significantly higher than expected when guessing. Hence, we seem to be successful at giving users coarse-grained information about the data.

\begin{figure}
\centering
\begin{tikzpicture}
\begin{axis}[width=8cm, height=3.5cm, ybar=0pt, legend entries={Voice, Visual}, legend columns=2, legend to name=prefLegend, ymajorgrids, xticklabels={U1, U2, U3, U4}, xtick={1,...,10},
  x tick label style={rotate=0}]
\addplot coordinates {(1,6) (2,8) (3,3) (4,7)};
\addplot coordinates {(1,7.5) (2,7) (3,9) (4,4)};
\end{axis}
\end{tikzpicture}

\ref{prefLegend}
\caption{User preferences comparing visual and voice interfaces (on site study).\label{onSitePreferences}}
\end{figure}

Figure~\ref{onSitePreferences} shows user preferences, a complementary metric. Participants were asked to rate the visual and the voice interface on a scale from one to ten. Here, the picture is more diverse. Participants were split on whether they preferred the voice or the visual interface. Among the reasons cited in support of voice interfaces were ease of access and reduced typing overheads. Among the reasons cited in support of the visual interface were a more detailed output and more reliable input recognition. The participant with highest preferences for the voice interface was also the least experienced SQL user (only based on course content). The participant with strongest preferences for the SQL interface was at the same time the most experienced SQL user. In addition, speech recognition did not work well in a large percentage of cases (which the participants himself linked to a strong accent). 

%In terms of desired improvements, three of our participants suggested improvements in user guidance (e.g., more explanations from the system about which data is available). Two participants considered the current query model sufficient while the others suggested extensions, in particular support for 


==> sections/model.tex <==

We introduce our problem model. Generally, our goal is to summarize rows in a relation via speech descriptions. First, we introduce scopes. 

\begin{definition}
A scope is defined by a set (i.e., conjunction) of unary equality predicates. We model scopes by a set of (column to value) assignment pairs. Hence, one scope $scp_1$ generalizes a second scope $scp_2$ if $scp_1\subseteq scp_2$. We say that relation rows lay within the scope of a query if they satisfy all scope predicates. We consider query scopes and fact scopes in the following. A query scope defines data that the user wants to access. A fact scope defines a data subset that a fact describes. We summarize scopes into scope groups. All scopes within a group place restrictions on the same set of relation columns. For a fixed relation, we characterize scope groups via column sets. The scope group contains one scope for each value combination that appears in the relation.
\end{definition}

We focus on high-level, exploratory data analysis (e.g., by lay users who want to get a quick impression about interesting trends in a data set). Our goal is not to support in-depth data analysis via complex queries. Hence, our query model is deliberately simple.

\begin{definition}
A user query is characterized by a target column as well as a query scope. The intent of the query is to obtain a speech summary of values in the target column, for rows within the query scope. 
\end{definition}

\begin{example}
For instance, users may ask about the salary in the United States. Here, the corresponding query scope is characterized by a restriction of the country column to the value ``United States''. The target column contains salary information. 
\end{example}

A query is answered by a speech summary. For our algorithms, we model speech summaries at a high level of abstraction. This model is introduced next.

\begin{definition}
A speech is a collection of facts. Each fact describes values in the target column for a specific scope (fact scope). We consider two types of facts. Typical value facts describe the average value in the target column within their fact scope. Range facts describe lower and upper value bounds. We require that each fact within a speech must have a fact scope specializing the query scope. This seems reasonable as it avoids burdening users with information outside of their query scope. With regards to a target column, we consider a fixed set of dimension columns that can be restricted for fact scopes. We restrict the maximal number of facts per speech and the maximal number of assignments per scope. Both is motivated by the limitations of listeners~\cite{MILLER1956, Trummer2018} in consuming spoken information. 
\end{definition}

We assume that users translate speech summaries into a mental model of the data. To compare speeches, we model the user's expectations after listening. We calculate speech quality based on how close user's expectations come to actual values. We assume that speeches either contain only typical value facts or only range facts. Next, we define user models for both types.

\begin{definition}
For speeches containing typical value facts, we assume a (domain and target-specific) value that users, in the absence of more specific information, default to. After listening to a speech, users change their estimates for rows that fall within fact scopes to the associated fact average value. Fact scopes may overlap, creating conflicting information. Optimistically, we assume that users will be able to identify the value that comes closest to the correct value among the alternatives (e.g., based on domain-specific knowledge about the relative importance of different factors). Denoting by $\mathcal{U}(s,r)$ the expectation of users about the target value in row $r$ after listening to speech $s$, we define the row error as $\mathcal{E}_T(s,r)=|\mathcal{U}(s,r)-r.tcol|$. We sum up row errors within an entire query scope, to assess how well a speech summarizes the associated data.
\end{definition}

\begin{example}
Reconsider the previous example. Users may expect an average salary of 50K in the United States (or, alternatively, they have been informed about the general average by initial speech output). Informing users that the salary for biologists in a small city named Ithaca is around 90K is not very useful to obtain a good overview of the data as a whole (as this fact refers to a small sub-population of the data). Also, informing users that the salary of high school teacher is around 48K is not very useful (as it changes the expectations only by little). Instead, it is more interesting to inform users that the average salary in the North-East of the United States is 70K. This fact applies to a relatively large data subset and the same time deviates enough from the general average to be interesting. Passing on that piece of information, decreases the expected estimation error a user makes when being asked to estimate salary for persons in specific areas with specific professions.
\end{example}

\begin{definition}
For speeches containing value range facts, we assume a default value range that is narrowed down via speech descriptions. Facts are combined with default expectations by intersecting all associated value ranges (each fact only applies to rows within its fact scope). The range error for a query scope after listening to a speech, is the sum of the distance between upper and lower range bounds over all rows within the scope.
\end{definition}

Our models are necessarily simplifying (as the human psyche is too complex to model accurately). However, we will show in our experiments that speeches selected according to our models enable users to answer questions about data with good precision. We are now ready to define the problem addressed in this paper.

\begin{definition}
Given a relation $R$ with target column $tcol$, a set of query scope groups $QSG$ and fact scope groups $FSG$, as well as a constraint on speech length $sl$ (maximal number of facts per speech), the goal of batch speech summarization is to find a speech for each query scope that minimizes error according to one of the two aforementioned metrics.
\end{definition}

Note that, for facts as well as for queries, we do not consider the power set of dimension columns. For instance, there are scenarios with a focus column that should appear in each fact (e.g., we consider a set of election results in our experiments where each fact should restrict by candidate). Also, data sets often have columns with specialization relationships between them (e.g., states and districts). In those cases, a restriction for the more specific category makes restricting the general one unnecessary. In the following, we propose exact and approximate algorithms for the optimization problem above.

With regards to the previous definitions, we use the following notations in our algorithms. Assuming a fixed target column, we denote by $r.tcol$ the value in the target column for a relation row $r$. Also, we denote by $r.dimValues$ the set of assignments from dimension columns to values that characterize row $r$. For each fact $f$, we denote by $f.scp$ the associated fact scope. Similarly, we denote by $s.scp$ the scope that a speech $s$ is summarizing. More notations are introduced as needed.

\begin{comment}

A user query on a relation designates a target column and a query scope. Our goal is to summarize values in the We summarize data in the target column. 

The demonstrated system uses the following (simple) query model, referring to data in one relation. A user query $q=\langle t,P\rangle$ is modeled by a combination of a target column $t$ and a predicate $P$. The predicate $P=\{\langle c,v\rangle\}$ is modeled as a set of column-value pairs modeling a conjunction of unary equality predicates. The goal of voice output is to describe the value distribution in the target column for all rows satisfying the predicate. 

Speech descriptions may refer to values in the target column as well as to values in dimension columns $D$ (a subset of columns that are suitable for forming voice descriptions). For a query $q$ on a relation $R$ with dimension columns $D$, function $F(R,q,D)$ denotes the set of facts suitable for voice descriptions. Facts include for instance statements about average values in the target column for specific value combinations in the dimension columns. Queries are answered via speeches that summarize a subset of facts: $s\subseteq F(R,q,D)$. Only a small set of facts can be spoken out without overwhelming listeners. The demonstrated system therefore tries to select the optimal combination of facts for output.

The goal is to give users the best possible approximation of the queried data. Denote by $\mathcal{A}(s)$ the approximation obtained by combining facts from speech $s$. Function $\mathcal{A}$ maps rows in the table the speech refers to, to an estimate for the associated value in the target column. The definition of the approximation function integrates the results of user studies on how listeners compose speech descriptions into a mental data model~\cite{Trummer2018a}. For a given row $r$ with target value $v$, we can define the error as $|\mathcal{A}(r)-v|$. This is the expected error made by users asked to estimate the target value in $r$. Denoting by $\mathcal{E}(q,s)$ the error sum over all rows within the scope of $q$, using the approximation created by speech $s$, the demonstrated system aims to select speech descriptions minimizing $\mathcal{E}(q,s)$ over all $s\subseteq F(q,R,D)$ such that $|s|\leq m$ (where $m$ designates the maximal number of facts per speech).
\end{comment}

==> sections/pruning.tex <==

Our goal is to make the greedy algorithm more efficient. We do so by reducing the number of facts that are considered as speech extensions. The version presented in the last section tries out all facts to optimally expand speeches. If we are able to prune groups of facts before generating them, efficiency can be improved. We present an approach to prune guaranteed sub-optimal fact groups in Section~\ref{factsSub}. 

Pruning fact groups can reduce execution time. On the other side, pruning introduces overheads that may not pay off. In this section, we present an optimizer generating pruning plans. We describe the cost model in Section~\ref{costSub}, define a plan space using heuristics in Section~\ref{plansSub}, and an optimization algorithm in Section~\ref{optimizerSub}.

\subsection{Fact Pruning}
\label{factsSub}

\begin{algorithm}[t]
\renewcommand{\algorithmiccomment}[1]{// #1}
\begin{algorithmic}[1]
\State \Comment{Use source facts $SFG$ to prune target facts $TFG$ for}
\State \Comment{relation $R$ and return fact groups from $FG$ that}
\State \Comment{remain interesting after explicit and implicit pruning}
\State \Comment{(considering current scopes $qsg$ and speeches $B$).}
\Function{PruneFGs}{$R,qsg,SFG,TFG,FG,B$}
\State \Comment{Worst approximation with source facts}
\State $w\gets errUB(R,qsg,B,SFG)$
\State \Comment{Calculate pruned target facts}
\State $P\gets\{t\in TFG\cap FG|errLB(R,qsg,B,\{t\})>w\}$
\State \Comment{Consider implicit pruning}
\State $I\gets \{g\in FG|\exists p\in P:p\subseteq g\}$
\State \Comment{Return remaining fact groups}
\State \Return{$FG\setminus (P\cup I)$}
\EndFunction
\vspace{0.15cm}
\State \Comment{Generate facts on data in $R$ within query scopes $qsg$}
\State \Comment{using fact scopes in $FSG$ and pruning plan $pp$. Only}
\State \Comment{consider facts that can optimally expand speeches $B$.}
\Function{GenerateFacts}{$R,qsg,FSG,pp,B$}
\State \Comment{Iterate over steps in pruning plan}
\For{$\langle SFG, TFG\rangle\in pp.steps$}
\State \Comment{Prune via specified source and target facts}
\State $FSG\gets$\Call{PruneFGs}{$R,qsg,SFG,TGF,FG,B$}
\EndFor
\State \Comment{Generate facts for pruned fact scope groups}
\State \Return{$\cup_{fsg\in FSG:qsg\subseteq fsg}(\Gamma_{fsg,avg(r.tcol)}(r\in R))$}
\EndFunction
\end{algorithmic}
\caption{Successively generate facts while pruning out dominated fact groups according to pruning plan.\label{pruningAlg}}
\end{algorithm}

Fact pruning is based on the following principle. We only prune fact groups that cannot contain any optimal facts. ``Optimal facts'' are facts that optimally expand the speech for at least one query scope. The optimal speech expansion minimizes approximation error. We introduce two functions that bound the error, achievable by expansion via specific fact groups. Let $qsg$ be the current query scope group, $B$ best speeches for those scopes, $FSG$ fact scope groups, and $R$ the relation. Function~$errUB(R,qsg,B,FSG)$ denotes maximal approximation error over all query scopes from $qsg$ when considering the following speeches. We consider speeches from $B$ that are optimally expanded by one fact from the fact scope groups in $FSG$. 

Function~$errLB(R,qsg,B,FSG)$ denotes an optimistic lower bound on the error over all query scopes, that can be achieved by adding facts from $FSG$. For a given fact, we obtain an optimistic bound on the error reduction as follows. We simply consider the current error for all rows within the fact scope, and assume that adding that fact reduces it to zero. The definitions of $errUB$ and $errLB$ are asymmetric: one ($errUB$) is more realistic, as it is based on error reduction by actual facts, the other one ($errLB$) is highly optimistic. The reasons behind this asymmetry will become clear later in this subsection. First, we discuss how those bounds are used for pruning.

Denote by $fsg_1$ and $fsg_2$ two fact scope groups. Assume that  $errUB(R,qsg,B,fsg_1)\leq errLB(R,qsg,B,fsg_2)$ (we omit set notation for singleton sets to simplify notation). In that case, $fsg_2$ can be pruned without regret. Considering facts from $fsg_1$ always yields more accurate speeches than considering facts from $fsg_2$ for any query scope. This pruning condition may seem restrictive. We only prune if the error of the best scope for one set of facts exceeds the error of the worst scope for another fact set. However, it is typically sufficient to avoid generating large groups of highly specific facts. Such facts describe only small data subsets and reduce overall approximation error only by little. It is often possible, to prune out such groups before generation, by comparing against error bounds for small groups of rather general facts. 

\begin{example}
Consider a data set summarizing flight delays. Fact groups referring to the season are likely to reduce approximation error significantly (as each season covers a large number of flights and as average delays will correlate). On the other side, facts referring to specific airports are probably too specific and reduce approximation error only little (as flights are partitioned over many airports). Hence, the technique presented before may allow us to avoid considering speech expansions by airport-related facts, based on error bounds for both fact groups.
\end{example}

Algorithm~\ref{pruningAlg} exploits that principle. It generates facts, while trying to prune out dominated fact groups early. It is invoked instead of the original \textproc{GenerateFacts} function (see Algorithm~\ref{auxBasicAlg}) in Algorithm~\ref{approxAlg}, using a slightly expanded set of invocation parameters. If pruning is used, facts need to be re-generated for each expansion (iterations of the inner-most loop) as formerly sub-optimal facts may become optimal later. To generate facts, Algorithm~\ref{pruningAlg} executes a pruning plan, defined next.

\begin{definition}
A pruning plan $pp$ describes the order in which facts are generated and, if possible, pruned. It is defined by an (ordered) sequence of steps, denoted by $pp.steps$. Each step is described by a pair $\langle SFG,TFG\rangle$. Both components denote sets of fact groups, we call $SFG$ the source fact groups and $TFG$ the target fact groups. Error bounds for source fact groups are used to prune the targets.
\end{definition}

Algorithm~\ref{pruningAlg} executes pruning plans as follows. We start with the full set of relevant fact scope groups, $FSG$. For each step of the pruning plan, Function~\textproc{PruneFSG} is invoked for pruning. Using bounds obtained via source fact groups, it identifies sub-optimal targets. We consider two types of pruning: explicit and implicit pruning. Explicit pruning happens if lower error bounds, calculated for a target group, exceed upper error bounds from the source. Implicit pruning exploits specialization relationships between target groups, described by the following theorem. 

\begin{theorem}
If fact group $src$ prunes $tar$, it implicitly prunes any specialization $spec$ of $tar$ with $tar\subseteq spec$.
\end{theorem}
\begin{proof}
If $src$ prunes $tar$ then $errUB(src)\leq errLB(tar)$ (we omit fixed parameters $R$, $qsg$, and $FSG$ to improve readability). However, $errLB$ is an optimistic bound, based only on the error sum within fact scopes. Specializing a fact further can only decrease that error sum. Hence, if $spec$ specializes $tar$ (i.e., $tar\subseteq spec$), we must have $errLB(spec)\geq errLB(tar)$. As $errUB(src)\leq errLB(tar)$, we must also have $errUB(src)\leq errLB(spec)$.
\end{proof}

Explicit pruning requires calculating accumulated error per fact scope for the target scope groups. In our SQL-based implementation, this is achieved by executing group by queries on the associated relation. On the other side, implicit pruning is based on a comparison between fact groups alone. It does not require issuing queries. Algorithm~\ref{pruningAlg} exploits both types of pruning. After pruning targets explicitly, it compares with the remaining fact scope groups for implicit pruning. Finally, Algorithm~\ref{pruningAlg} generates facts in groups that were not pruned out. Note that the pseudo-code is slightly simplified by omitting caching-related instructions. E.g., if an upper error bound was calculated for a fact group, the corresponding facts must have been generated. The actual implementation avoids re-generating facts, the code extension is natural. 

Algorithm~\ref{pruningAlg} depends on the selection of a pruning plan. We show in Section~\ref{experimentsSec} that pruning, if not used carefully, can hurt performance. Next, we discuss a cost model that allows to compare (and to optimize) pruning plans.

\subsection{Cost Model}
\label{costSub}

We denote by $Pcost(pp)$ the (estimated) execution cost of a pruning plan $pp$. The cost of a plan is the sum of the execution costs of each plan step $pp_i$: \[Pcost(pp)=\sum_{i}Scost(pp_i,\{pp_j|1\leq j\leq i-1\})\]. The cost of each step does not only depend on the step itself but also on prior steps in the plan. Each plan step $\langle src,tar\rangle$ specifies a pruning operation that compares error bounds for source scopes $src$ to target scopes $tar$. However, some of the target scopes may have been (implicitly or explicitly) pruned by previous steps. The same applies for source scopes. If so, the current step becomes cheaper.

For a given plan, denote by $src_i$ and $tar_i$ the source and target scopes used for the $i$-th plan step. Function $Ecost(sg)$ denotes the cost of calculating error bounds for scope group $sg$. We simplify our cost model by assuming that calculating lower and upper error bounds (i.e., Functions~$errUB$ and $errLB$) have the same cost function. The expected cost of the $i$-th plan step is then given as \[\sum_{sg\in src_i\cup tar_i}\Pr(\text{$sg$ not pruned before})\cdot Ecost(sg)\]. 

Scope groups may be pruned explicitly if they appear as target scopes in prior steps. Also, they may be pruned implicitly if they specialize scopes that were previously pruned. A scope group remains relevant if none of its generalizing scopes were previously pruned. Hence, denoting by $psrc=\cup_{1\leq j\leq i-1}src_i$ and $ptar=\cup_{1\leq j\leq i-1}tar_i$ previous sources and targets respectively, we obtain 
\begin{align*}
&\Pr(\text{$sg$ not pruned})\\
=&\Pr(\nexists t\in ptar:t\subseteq sg,\text{$t$ was pruned})\\
=&\Pr(\nexists s\in psrc,t\in ptar:t\subseteq sg,\text{$s$ prunes $t$})
\end{align*}

for the $i$-th plan step. We simplify by assuming independence between different pruning outcomes. Then, we obtain
\begin{align*}
\Pr(\text{$sg$ not pruned})=\prod_{s\in psrc}\prod_{t\in ptar:t\subseteq sg}(1-\Pr(\text{$s$ prunes $t$}))
\end{align*}

Still, we need to calculate the probability that error bounds, obtained for one scope group, dominated others. We aggregate error for a scope by summing up over all rows within it. Hence, assuming a uniform distribution of error over rows, the error should correlate with scope size. Furthermore, we assume a normal distribution to model error for specific scopes. This seems reasonable based on the following perspective. If we consider the per-row errors as identical, independently distributed random variables, the error approaches a normal distribution due to the Central Limit theorem. 

During pruning, we compare two scope groups. We compare the minimum error over all scopes in the first group against the maximal error over all scopes in the second group. As discussed before, we assume that per-scope error follows a normal distribution. We simplify by assuming that each scope in a group accumulates the same error. This is justified if rows are distributed uniformly over scopes for each scope group, and if the per-scope error varies little. As we assume having the same error for each scope, error minima and maxima collapse. Hence, when comparing two scope groups $s$ and $t$ with sizes (i.e., number of scopes) $nsc_1$ and $nsc_2$, we introduce random variable $E\sim\mathcal{N}(err/nsc_1-err/nsc_2,\sigma^2)$ (where $err$ and $\sigma^2$ are constants, representing the accumulated error over all rows and the error variance respectively) and obtain\[\Pr(\text{$s$ prunes $t$})=\Pr(\text{$E\leq 0$})\]. The number of scopes in each scope group is determined by the number of unique value combinations in the scope group columns. Hence, it can be estimated via data statistics, typically maintained by relational DBMS (we leverage statistics of the Postgres database system in our implementation). 

Our cost model for pruning plans is simplifying. However, our goal is not to estimate precise cost. Our goal is to establish a relative ranking among plans to select a near-optimal one. In our experiments, we show that this model is sufficient for that purpose.

\subsection{Plan Space}
\label{plansSub}

A-priori, the search space for pruning plans is large (we re-use the notations from Section~\ref{exactComplexitySub} in the following). 

\begin{lemma}
There are $\Omega(sgs!\cdot 2^{sgs})$ pruning plans.
\end{lemma}
\begin{proof}
We obtain upper error bounds for source scopes, and upper error bounds for target scopes. Those bounds remain unchanged over different plan steps. Hence, there is no need to include the same scopes twice as source or target in the same plan. For a valid pruning plan, the union of source scopes over different steps needs to cover all scopes. Each plan step needs to contain at least one new source scope (otherwise, consecutive plan steps could be merged without changing cost). Hence, we have $O(sgs)$ plan steps. We can choose the order in which source scopes are added and partition them into $O(sgs)$ plan steps. Independently of the choice of target scopes, each possible order and partition leads to a different pruning plan. There are $O(sgs!)$ possible orders and $O(2^{sgs})$ ways to partition a given order into steps (we choose for each scope group whether it is added in a new step or in the current one). 
\end{proof}

This bound can be tightened. However, it already shows that naively exploring all possible pruning plans is too expensive. We apply several heuristics to focus on a subset of interesting plans during optimization (we will discuss results for more general pruning plans in Section~\ref{experimentsSec} as well). 

\begin{heuristic}
Add source scope groups in ascending order of scope count.\label{nrScopesHeuristic}
\end{heuristic}

This heuristic is motivated by the following insight. According to the cost model described in the previous subsection, a scope group is more likely to prune out others (in a comparison) if it contains less scopes. If we use strong pruning sources earlier in the plan, this may enable us to prune out other scope groups earlier (thereby minimizing cost).

\begin{heuristic}
We consider plans with a bounded number of pruning steps (bounded by a constant).
\end{heuristic}

Each step in a pruning plan adds overheads (since we need to calculate error bounds). As the number of steps increases, pruning overheads will start to rival cost savings for generating facts. In our experience, fact pruning is most useful if one group of very generic facts exists that can prune a large percentage of other fact groups. This can be achieved with one single pruning step. 


%This heuristic may seem particularly restrictive. If a pruning plan has no steps, it means that we do not use any pruning. This means that all facts are generated. On the other side, we avoid pruning-related overheads for calculating error bounds. As demonstrated in Section~\ref{experimentsSec}, avoiding any pruning can be the most efficient alternative. If a pruning plan has one step, we calculate upper error bounds for source scopes. Then, we use them to prune target scopes based on their (lower) error bounds. We generate facts for all remaining scopes.

%Pruning saves cost for calculating upper error bounds if source scopes are pruned. It saves cost for calculating lower error bounds if target scopes are pruned. Finally, it saves cost by reducing the number of facts that are finally generated. 


\subsection{Optimization Algorithm}
\label{optimizerSub}

\begin{algorithm}[t]
\renewcommand{\algorithmiccomment}[1]{// #1}
\begin{algorithmic}[1]
\State \Comment{Construct optimal pruning plan for generating facts}
\State \Comment{using fact scope groups in $FSG$.}
\Function{FGoptimizer}{$FSG$}
\State \Comment{Initialize pruning plan candidates}
\State $PP\gets\emptyset$
\State \Comment{Order fact scope groups by estimated size}
\State $fsg_1,\ldots,fsg_m\gets$ $FSG$ groups by size (ascending)
\State \Comment{Iterate over size for pruning source}
\For{$srcs\gets1,\ldots,m$}
\State \Comment{Collect fact groups as pruning source}
\State $src\gets \cup_{1\leq i\leq srcs}\{fsg_i\}$
\State \Comment{Collect candidates for pruning target}
\State $tcand\gets \cup_{srcs+1\leq i\leq m}\{fsg_i\}$
\State \Comment{Initialize pruning target}
\State $tar\gets\emptyset$
\State \Comment{While pruning candidates left}
\While{$tcand\neq\emptyset$}
\State \Comment{Select next pruning target}
\State $t\gets\arg\max_{c\in tcand}\mathbb{E}(\text{nr pruned}|src,c)$%\Pr(\text{$t$ pruned}|src)\textproc{Tpruned}(src,c,tcand)$
\State \Comment{Add to set of pruning targets}
\State $tar\gets tar\cup\{t\}$
\State \Comment{Take into account implicit pruning}
\State $tcand\gets tcand\setminus\{c\in tcand|tar\subseteq c\}$
\State \Comment{Construct and add corresponding plan}
\State $PP\gets PP\cup\{$\Call{PPlan}{$src,tars$}$\}$
\EndWhile
\EndFor
\State \Comment{Select pruning plan with minimal cost}
\State \Return{$\arg\min_{pp\in PP}Pcost(pp)$}
\EndFunction
\end{algorithmic}
\caption{Generate plan determining how fact groups are generated and pruned.\label{optimizerAlg}}
\end{algorithm}

We discuss an algorithm that explores the search space of pruning plans (restricted as discussed in the previous section). Algorithm~\ref{optimizerAlg} shows corresponding pseudo-code. The function first orders fact scope groups by scope count. Next, the function iterates over the number of fact groups to use as source in the first pruning step. We use the fact scope groups with the lowest number of scopes as source (Heuristic~\ref{nrScopesHeuristic}). The remaining fact scope groups are used as candidate pruning targets. We add pruning targets greedily, maximizing in each step the expected number of pruned groups (using the model presented in Section~\ref{costSub} and considering implicit as well as explicit pruning). After adding a pruning target, we remove other targets that are implicitly pruned by the latest addition from the candidate set. For a fixed number of source scope groups and target scope groups, we add a corresponding pruning plan to the set of considered plans. Finally, we return the pruning plan with minimal estimated cost according to the model from Section~\ref{costSub}. Note that we describe the pseudo-code for the case of single-step pruning plans. The generalization to bounded length pruning plans is natural (it requires adding one more nested loop, iterating over the number of plan steps). In practice, we found single step pruning plans to work well for our benchmarks.


%Algorithm~\ref{optimizerAlg} specifically explores the space of single step pruning plans. We found such plans to offer already a good tradeoff between pruning overheads and benefit. We found such pruning plans to be sufficient in practice. 

\begin{comment}
\begin{align*}
&\textproc{Tpruned}(src,c,tcand)\\
=&\Pr(\exists s\in src:\text{$s$ dominates $c$})\cdot \textproc{Ipruned}(c,tcand)\\
\end{align*}

\begin{align*}
\textproc{Ipruned}(c,tcand)=|\{t\in tcand|c\subseteq t\}|
\end{align*}

\begin{align*}
&\Pr(\exists s\in src:\text{$s$ dominates $c$})\\
=&\prod_{s\in src}\Pr(\text{$s$ dominates $c$})
\end{align*}

\begin{align*}
&\Pr(\text{$s$ dominates $c$})\\
=&\Pr(err(s)<err(c))
\end{align*}

\begin{equation*}
err(s)\sim\mathcal{N}(1/\textproc{Nfacts}(s),\sigma^2)
\end{equation*}
\end{comment}
